Compositional Reinforcement Learning from Logical Specifications

We study the problem of learning control policies for complex tasks given by logical specifications. Recent approaches automatically generate a reward function from a given specification and use a suitable reinforcement learning algorithm to learn a policy that maximizes the expected reward. These approaches, however, scale poorly to complex tasks that require high-level planning. In this work, we develop a compositional learning approach, called DiRL, that interleaves high-level planning and reinforcement learning. First, DiRL encodes the specification as an abstract graph; intuitively, vertices and edges of the graph correspond to regions of the state space and simpler sub-tasks, respectively. Our approach then incorporates reinforcement learning to learn neural network policies for each edge (sub-task) within a Dijkstra-style planning algorithm to compute a high-level plan in the graph. An evaluation of the proposed approach on a set of challenging control benchmarks with continuous state and action spaces demonstrates that it outperforms state-of-the-art baselines.

==> Section/algo.tex <==
In this section, we propose a compositional approach for learning a policy to solve the abstract reachability problem for MDP $\M$ and abstract graph $\G$.

At a high level, our algorithm proceeds in three steps:
\begin{itemize}[topsep=0pt,itemsep=0ex,partopsep=1ex,parsep=1ex]
\item For each edge $e=u\to u'$ in $\G$, use RL to learn a neural network (NN) policy $\pi_e$ to try and transition the system from any state $s\in u$ to some state $s'\in u'$. Importantly, this step requires devising a distribution $\eta_u$ over initial states $s\in u$.
\item Use sampling to estimate the probability $P(e;\pi_e,\eta_u)$ that $\pi_e$ successfully transitions from $u$ to $u'$.
\item Use Djikstra's algorithm in conjunction with the edge costs $c(e)=-P(e;\pi_e,\eta_u)$ to compute the path $\rho^*=u_0\to u_1\to\cdots\to u_k$ in $\G$ that minimizes
\begin{align*}
c(\rho)=\prod_{i=0}^{k-1}P(e_i;\pi_i,\eta_i),
\end{align*}
where $e_i=u_i\to u_{i+1}$, $\pi_i=\pi_{e_i}$, and $\eta_i=\eta_{u_i}$.
\end{itemize}
Then, we could choose $\pi$ to be the sequence of policies $\pi_1,...,\pi_{k-1}$---i.e., execute each policy $\pi_i$ until it reaches $u_{i+1}$, and then switch to $\pi_{i+1}$.

There are two issues with this approach. First, it is unclear what distribution to use as the initial state distribution $\eta_u$ to train $\pi_e$.
%how to sample start states for training these policies since the distribution over states in a source subgoal region depends on the learned policies as well as the high level plan. 
Second, it might be unnecessary to learn all the policies since a subset of the edges might be sufficient for the reachability task. Our algorithm (Algorithm~\autoref{alg:dijkstra}) addresses these issues by lazily training $\pi_e$---i.e., only training $\pi_e$ when the edge cost $c(e)$ is needed by Djikstra's algorithm.
%by learning a policy corresponding to an edge only when the cost of the edge is queried by the planning algorithm.

\subsection{The \dirl Algorithm}

Our algorithm
%(Algorithm~\ref{alg:dijkstra}) optimizes (\ref{eqn:obj}) by
interleaves Djikstra's algorithm with using RL to train policies $\pi_e$. It runs Djikstra's algorithm with
\begin{align*}
c(e)=-\log P(e;\pi_e,\eta_u)
\end{align*}
as the cost for edge $e=u\to u'$,\footnote{Note that we take the negative logarithm since Djikstra's algorithm computes the path with minimum summed edge weights.}
computing edge weights on-the-fly by training a policy $\pi_e$ for $e$, and then using Monte Carlo estimation to estimate it. Note that $c(e)$ is always nonnegative for any edge $e$.

%\textbf{State distributions.}
%%
%As described above, the main issue with this approach is what to choose for $\eta_u$. To address this issue, our algorithm keeps track of the path policy $\tilde{\pi}_u$ for transitioning the system from $u_0$ to $u$ with the highest success probability $P(\tilde{\pi})$. Then, it chooses $\eta_u=\eta_{\tilde{\pi}_u}$ to be the state distribution induced by using $\tilde{\pi}_u$.

In more detail, \dirl iteratively processes subgoal regions $u$ in $\G$ starting from the initial region $u_0$, and continuing until it processes a final subgoal region $u\in F$. It maintains the property that for every $u$ it processes, it has already trained policies for all edges along some path $\rho_u$ from $u_0$ to $u$.
%at least one path policy $\tilde{\pi}_u$ with final subgoal region $u$.
This property is satisfied by $u_0$ since there is a path of length zero from $u_0$ to itself.
%for the singleton path policy $u_0$ (this policy does not do anything since any state $s\sim\eta$ satisfies $s\in u_0$ by definition of $u_0$).
In Algorithm~\ref{alg:dijkstra}, $\Gamma_u$ is the set of all paths from $u_0$ to $u$ discovered so far, and $\Pi = \{\pi_e\mid e\in E\}$ is the set of all edge policies constructed so far.

In each iteration, \dirl processes the unprocessed subgoal region $u$ nearest to $u_0$, and performs the following steps:
\begin{enumerate}[topsep=0pt,itemsep=0ex,partopsep=1ex,parsep=1ex]
\item Select the shortest path from $u_0$ to $u$ in $\Gamma_u$, denoted
\begin{align*}
\rho_u=u_0\to\cdots\to u_k=u.
\end{align*}
\item Compute the distribution $\eta_u$ over states in $u$ induced by using the sequence of policies $\pi_{e_1},...,\pi_{e_{k-1}}\in\Pi$, where $e_i=u_i\to u_{i+1}$ are the edges in $\rho_u$.
\item For every edge $e=u\to u'$ in $\G$, learn a policy $\pi_e$ for the $e$ using $\eta_u$ as the initial state distribution, and add
\begin{align*}
\rho_{u'}=u_0\to\cdots\to u\to u'
\end{align*}
to $\Gamma_{u'}$ and $\pi_e$ to $\Pi$.
\end{enumerate}

\begin{algorithm}[tb]
\caption{Compositional learning for abstract reachability.}
\label{alg:dijkstra}
\begin{algorithmic}
\FUNCTION{\dirl($\G$)}
%\STATE Initialize policies $\pi_e$ for $e\in E$ and $\pi_u$ for $u\in F$
%\STATE Initialize state distributions $\eta_u$
\STATE Initialize processed subgoal regions $U_p\gets\varnothing$
\STATE Initialize $\Gamma_{u_0}\gets\{u_0\}$, and $\Gamma_u\gets\varnothing$ for $u\neq u_0$
\STATE Initialize edge policies $\Pi\gets\varnothing$
%\STATE Initialize policies $\pi_e$ for $e\in E$
%\STATE Set $c_u \gets \infty$ for every $u\in U\setminus\{u_0\}$
%\STATE Set $c_{u_0}\gets 0$
\WHILE{\textbf{true}}
\STATE $u \gets \textsc{NearestRegion}(U\setminus U_p, \Gamma, \Pi)$
\STATE $\rho_u\gets\textsc{ShortestPath}(\Gamma_u)$
\STATE $\eta_u\gets\textsc{ReachDistribution}(\rho_u,\Pi)$
\IF{$u\in F$}
%\STATE $\pi_u \gets \text{LearnFinalPolicy}(u, \eta_u)$
\STATE \textbf{return} $\textsc{PathPolicy}(\rho_u,\Pi)$
\ENDIF
\FOR{$e = u \to u' \in \text{Outgoing}(u)$}
\STATE $\pi_e \gets \textsc{LearnPolicy}(e, \eta_u)$
\STATE Add $\rho_u\circ e$\ to\  $\Gamma_{u'}$
\STATE Add $\pi_e$ to $\Pi$
%\STATE Let $c'_{u_2} = c_{u_1} - \log(P(u_1\to u_2;\eta_{u_1}))$
%\IF{$c'_{u_2} < c_{u_2}$}
%\STATE $c_{u_2}\gets c'_{u_2}$
%\STATE $\eta_{u_2}\gets \eta[u_1\to u_2,\eta_{u_1}]$
%\ENDIF
\ENDFOR
\STATE Add $u$ to $U_p$
\ENDWHILE
\ENDFUNCTION
\end{algorithmic}
\end{algorithm}

% \textbf{Step 1.}
% %
% It first chooses a single path $\tilde{\rho}_u$ to represent $u$---in particular, the one with the lowest cost:
% \begin{align*}
% \tilde{\pi}_u&=\operatorname*{\arg\min}_{\tilde{\pi}\in\Pi_u}c(\tilde{\pi}),\qquad
% c(\tilde{\pi})=-\log P(\tilde{\pi}).
% \end{align*}
% The quantities $P(e_i;\pi_i,\eta_i)$ in $P(\tilde{\pi})$ are estimated as described in Section~\ref{sec:estimate}. Furthermore, it lets $\eta_u=\eta_{\tilde{\pi}_u}$ be the state distribution induced by using $\tilde{\pi}_u$.
% %Intuitively, $\eta_u$ is the distribution of states induced by using the sequence of policies $\pi_i$ in $\tilde{\rho}_u$.
% %To address this issue, our algorithm keeps track of the path policy $\tilde{\pi}_u$ for transitioning the system from $u_0$ to $u$ with the highest success probability $P(\tilde{\pi})$. Then, it chooses $\eta_u=\eta_{\tilde{\pi}_u}$ to be the
% %The one exception is the initial vertex $u_0$, for which we take $\eta_{u_0}=\eta$ to be the initial state distribution of $\M$.
% At this point, if $u\in F$, then our algorithm returns $\tilde{\pi}_u$.

% \textbf{Step 2.}
% %
% It queries the cost of every edge $e=u\to u'$ for every neighbor $u'$ of $u$---i.e.,
% \begin{align*}
% e\in\text{Outgoing}(u) = \{e\in E\mid \exists u'\;.\; e=u\to u'\}.
% \end{align*}
% For every such edge $e$, it trains a policy $\pi_e$ using RL with $\eta_u$ as described in Section~\ref{sec:learning}. Then, it constructs a new path $\tilde{\pi}'$ to $u'$ that is $\tilde{\pi}_u$ concatenated with $u\xrightarrow{\pi_e}u'$---i.e.,
% \begin{align*}
% \tilde{\pi}'=\tilde{\pi}_{u}\circ(\pi_e,u')=u_0\xrightarrow{\pi_0}\cdots\xrightarrow{\pi_{k-1}}u\xrightarrow{\pi_e}u'.
% \end{align*}
% Then, it adds $\tilde{\pi}'$ to $\Pi_{u'}$.

% \textbf{Processing order.}
% %
% Finally, our algorithm chooses the next subgoal region $u$ to process to be the one that has not yet been processed, but has the lowest possible cost out of all its augmented paths---i.e.,
% \begin{align*}
% u=\operatorname*{\arg\min}_{u'\in U_p}\min_{\tilde{\pi}\in\Pi_{u'}}c(\tilde{\pi}).
% \end{align*}

We now describe each subroutine in detail.

\subsection{Learning an Edge Policy 
(\textsc{LearnPolicy})}

%\textbf{\textsc{LearnPolicy}.}
%\label{sec:learning}
%\textbf{Learning a single edge.}
%
%We have one neural network policy for every edge $(u_1,u_2)$ in the abstract graph which is to be trained to transitions the system from any state in the source subgoal region $u_1$ to the target subgoal region $u_2$.
First, we describe how \dirl learns a policy $\pi_e$ for a single edge $e=u\to u'$, assuming the initial state distribution $\eta_u$ is given. At a high level, it trains $\pi_e$ using a standard RL algorithm, where the rewards are designed to encourage $\pi_e$ to safely transition the system to $u'$.
%$\mathbbm{1}(s\in u')$ {\color{red} This should be $\mathbbm{1}(\zeta\models e)$ since safety is also needed}.
\begin{definition}
\rm
A rollout $\zeta = s_0\to\cdots\to s_t$ \emph{achieves} edge $e = u\to u'$ in $\G$ (denoted $\zeta\models e$) if (i) $s_0\in u$, and (ii) there exists $i \leq t$ such that $s_i\in u'$ and $\zeta_{0:i}\in\traj_{\safe}^e$; we denote the smallest such $i$ by $i(\zeta,e)$.
\end{definition}
That is, $\zeta$ safely reaches $u$. Then, the rewards used for learning are $\mathbbm{1}(\zeta\models e)$. Then, \textsc{LearnPolicy} uses a standard RL algorithm to compute $\pi^*_e = \operatorname*{\arg\max}_{\pi}P(e;\pi, \eta_u)$, where
\begin{align*}
P(e;\pi,\eta_u)=\Pr_{s_0\sim\eta_u,\zeta\sim\mathcal{D}_{\pi,s_0}}[\zeta\models e]
\end{align*}
is the probability that $\pi$ achieves $e$ from an initial state $s_0\sim\eta_u$. Here, $\mathcal{D}_{\pi,s_0}$ is the distribution over rollouts induced by using $\pi$ from initial state $s_0$. Shaped rewards can be used to improve learning; see Appendix~\ref{Ap:shaped_rewards} in the supplement.

\subsection{Constructing a Path Policy
(\textsc{PathPolicy})}

Given edge policies $\Pi$ along with a path
\begin{align*}
\rho=u_0\to u_1\to \cdots\to u_k = u,
\end{align*}
in $\G$, our algorithm constructs a \emph{path policy} $\tilde{\pi}_{\rho}$ to navigate from $u_0$ to $u$. In particular, $\tilde{\pi}_{\rho}$ executes $\pi_{u_i\to u_{i+1}}$ (starting from $i=0$) until reaching $u_{i+1}$, after which it increments $i\gets i+1$ (unless $i=k$). That is, $\tilde{\pi}_{\rho}$ is designed to achieve the sequence of edges in $\rho$. Note that $\tilde{\pi}_{\rho}$ is stateful since it internally keeps track of the index $i$ of the current policy.

\dirl returns a path policy from the initial subgoal region $u_0$ to a final subgoal region $u\in F$. For clarity, we have omitted what happens after reaching a final state $u\in F$. In our implementation, we additionally learn a policy $\pi_u$ for $u$ that safely keeps the system inside $u$.

\subsection{Initial State Distribution
(\textsc{ReachDistribution})}

\dirl chooses the initial state distribution $\eta_u$ for $u$ to be the distribution of states $\eta_{\rho_u}$ reached by $\tilde{\pi}_{\rho_u}$ from a random initial state $s_0\sim\eta$, where $\rho_u$ is the path from $u_0$ to $u$ that \dirl chooses when processing $u$. This choice is the distribution of states reaching $u$ by the path policy $\tilde{\pi}_{\rho}$ eventually returned by \dirl. Thus, it ensures that the training and test distributions for edge policies in $\tilde{\pi}_{\rho}$ are equal.

More precisely, given a path $\rho=u_0\to\cdots\to u_k$ and edge policies $\Pi$, the distribution $\eta_{\rho}$ is defined inductively on the length of the path $\rho$. For the zero length path $\rho = u_0$, we define $\eta_{\rho} = \eta$, the initial state distribution of the MDP $\M$.

Otherwise, we have $\rho = \rho'\circ e$, where $e = u'\to u$; then, we define $\eta_{\rho}$ to be the state distribution over $u$ induced by using $\pi_e$ from $s\sim\eta_{\rho'}$ conditioned on $\zeta\models e$. Formally, $\eta_{\rho}$ is the probability distribution over $u$ such that for a set of states $S'\subseteq u$, the probability of $S'$ according to $\eta_{\rho}$ is
\begin{align*}
\Pr_{s\sim\eta_{\rho}}[s\in S'] = \Pr_{s_0\sim\eta_{\rho'}, \zeta\sim\mathcal{D}_{\pi_e, s_0}}\left[s_{i(\zeta,e)}\in S'\mid \zeta\models e\right].
\end{align*}

\subsection{Shorest Path Computation
(\textsc{ShortestPath})}

%We define the cost of a path $\rho=u_0\to\cdots\to u_k=u$ as follows. Let $\rho_{i} = u_0\to\cdots\to u_i$ denote the prefix of $\rho$ of length $i$. Then, the cost of the path $\rho$ is
The cost of a path $\rho=u_0\to\cdots\to u_k=u$ is
\begin{align*}
c(\rho) = -\sum_{i=0}^{k-1}\log P(e_i;\pi_{e_i},\eta_{\rho_{0:i}})
\end{align*}
where $e_i = u_i\to u_{i+1}$ is the $i$th edge in the path $\rho$. Now, this subroutine returns the path of minimum cost
\begin{align*}
\tilde{\rho}_u = \operatorname*{\arg\min}_{\rho\in\Gamma_u}c(\rho).
\end{align*}
These costs can be estimated using Monte Carlo sampling. 
Finally, we have the following guarantee.
\begin{theorem}
\label{thm:main}
Given a path policy ${\pi_{\rho}}$ corresponding to a path $\rho = u_0\to\cdots\to u_k = u\in F$ we have
\begin{align*}
c(\rho) \ge -\log\Pr_{\zeta\sim\D_{{\pi_{\rho}}}}[\zeta \models \G].
%\prod_{i=0}^{k-1}P(e_i;\pi_{e_i},\eta_{\rho_i})
%%\cdot P(u_k;\pi_k,\eta_k).
\end{align*}
%where $e_i = u_i\to u_{i+1}$.
\end{theorem}
In other words, we guarantee that the cost function minimized by Algorithm~\ref{alg:dijkstra} is an upper bound on the minimization objective of the abstract reachability problem.

\subsection{Processing Order (\textsc{NearestRegion})}

On each iteration, \dirl chooses the subgoal region $u$ to process next to be the unprocessed region that has the shortest known path from $u_0$---i.e.,
\begin{align*}
u = \operatorname*{\arg\min}_{u'\in U\setminus U_p}\operatorname*{\min}_{\rho\in\Gamma_{u'}}c(\rho).
\end{align*}
This choice is an important part of Djikstra's algorithm. For a graph with fixed costs, it ensures that the computed path $\rho_u$ to each vertex $u$ is minimized. While the costs in our setting are not fixed since they depend on $\eta_u$, this strategy remains an effective heuristic.
%
%Given a rollout $\zeta\sim\mathcal{D}_{\tilde{\rho}}$ (where $\mathcal{D}_{\tilde{\rho}}$ is the distribution of rollouts generated by $\tilde{\rho}$), we can implicitly decompose $\zeta$ into segments $\zeta_{i_j:(i_{j+1}-1)}$ (where $0=i_0<...<i_h\le T$) such that $\zeta_{i_j}$ is the step at which $\tilde{\rho}$ increments $i\gets i+1$. Note that we have $h<k$ if $\zeta$ does not reach $u_k$.
% \begin{definition}
% \rm
% A rollout $\zeta$ generated using a path policy ${\pi_{\rho}}$ \emph{achieves} the path $\rho$ (denoted $\zeta\models\rho$) if each policy $\pi_i$ in $\tilde{\pi}$ achieves its corresponding edge $e_i$.
% \end{definition}
% We let $P(\pi_{\rho})=\Pr_{\zeta\sim\mathcal{D}_{{\pi_{\rho}}}}[\zeta\models\rho]$ be the probability that a rollout $\zeta$ generated using $\pi_{\rho}$ achieves $\rho$. Then, the cost for a path $\rho$ is given by
% \begin{align*}
%     c(\rho) = -\log(P(\pi_{\rho})).
% \end{align*}



% That is, the probability of achieving $\rho$ decomposes into the probabilities of achieving each edge. This property follows since the probability $\pi_i$ achieves $e_i$ is independent of the previous edges conditioned on $\pi_j$ achieving $e_j$ for all $j<i$.

% Finally, given a path policy $\tilde{\pi}$, we have
% \begin{align*}
% \Pr_{\zeta\sim\D_{\tilde{\pi}}}[\zeta \models \G] = P(\tilde{\pi}).
% \end{align*}
% Thus, Theorem~\ref{thm:main} gives us a formula for computing $\Pr_{\zeta\sim\D_{\tilde{\pi}}}[\zeta \models \G]$ (or at least estimate it using Monte Carlo). In particular, to optimize $\Pr_{\zeta\sim\D_{\tilde{\pi}}}[\zeta \models \G]$, it suffices to optimize the objective in Theorem~\ref{thm:main}:
% \begin{align}
% \label{eqn:obj}
% \pi^*=\operatorname*{\arg\max}_{\tilde{\pi}}\prod_{i=0}^{k-1}P(e_i;\pi_i,\eta_i).
% %\cdot P(u_k;\pi_k,\eta_k).
% \end{align}

%Then, a potential approach would be to train all these policies first and then use a high level planning algorithm to compute a path in the abstract graph.

% \subsection{Estimating Success Probabilities}
% \label{sec:estimate}

% Next, we describe how our algorithm estimates the success probability of $\pi_e$ given $\eta_u$---i.e., the probability

% Then, our algorithm estimates $P(e;\pi_e,\eta_u)$ using Monte Carlo estimation---i.e., (i) take $n$ random samples $s_0^{(i)}\sim\eta_u$ and $\zeta^{(i)}\sim\mathcal{D}_{\pi_e,s_0}$ for $i\in\{1,...,n\}$, (ii) compute $\delta^{(i)}=\mathbbm{1}(\zeta^{(i)}\models e)$, and (iii) use
% %\begin{align*}
% $P(e;\pi_e,\eta_u)\approx\frac{1}{n}\sum_{i=1}^n\delta^{(i)}$.
% %\end{align*}



%The terminal safety probability is
%\begin{align*}
%\Pr[\safe(u)\mid \eta_u] = \Pr_{s\sim\eta_k,\zeta\sim\D_{\pi_{u}}}[\zeta\in\traj_{\safe}^{u}\mid s_0 = s].
%\end{align*}


%A high level plan is simply a path from the initial subgoal region to a final subgoal region. Given a high level plan $\rho = u_0\to\cdots\to u_k$ we can define a policy $\pi$ for the underlying MDP which initially uses $\pi_{u_{0}\to u_1}$ and follows the current policy until its target subgoal region is reached after which the policy corresponding to the next edge is followed.

%\textbf{Compositional correctness.}
%
%Next, we show that the cost function we use in Djikstra's algorithm is a lower bound on the true cost (ignoring errors in our Monte Carlo estimates).
%Let $\Theta$ be the combined parameter space of all the NN policies $\pi_e$ for $e\in E$ and $\pi_u$ for $u\in F$. Given $\theta\in\Theta$ and a high level plan $\rho$, the resulting policy is denoted $\pi_{\theta}^{\rho}$. Since the set of policies defined compositionally is included in the set of all possible policies we have the following corollary.
%\begin{corollary}
%\begin{align*}
%\max_{\pi}&\Pr_{s\sim\eta, \zeta\sim\D_{\pi}}[\zeta\models \G\mid s_0=s]
%\geq \max_{\theta\in\Theta, \rho}\Pr_{\zeta\sim\mathcal{D}_{\tilde{\pi}}}[\zeta\models\rho]
%\Pr[\rho]\cdot\Pr[\safe(u_k)\mid\eta_k].
%\end{align*}
%\end{corollary}

%\subsection{Constructing Initial State Distributions}

%Next, we describe how our algorithm constructs the initial state distribution $\eta_u$ for subgoal regions to use when training $\pi_e$ to achieve edge $e=u\to u'$. 

%Then, we choose $\eta_u$ to be the state distribution over $u$ induced by using $\tilde{\pi}$ from $s\sim\eta$ conditioned on $\zeta\models\rho$, where $\eta$ is the initial state distribution of $\M$.
%%along with the policies $\pi_i$ learned for edges $e_i$ in $\rho$.
%\begin{definition}
%\label{def:induceddistribution}
%\rm
%Given a path policy $\tilde{\pi}$ whose final subgoal region is $u$, the \emph{induced state distribution} $\eta_{\tilde{\pi}}$ is the probability distribution over $u$ such that for a set of states $S'\subseteq u$, the probability of $S'$ according to $\eta_{\tilde{\pi}}$ is defined to be
%\begin{align*}
%\Pr_{s\sim\eta_{\tilde{\pi}}}[s\in S'] = \Pr_{\zeta\sim\mathcal{D}_{\tilde{\pi}}}\left[s_{i(\zeta,e)}\in S'\mid \zeta\models e\right].
%\end{align*}
%\end{definition}
%In other words, $\eta_{\tilde{\pi}}$ is the state distribution induced by using the path policy $\tilde{\pi}$ for $u$ from $s_0\sim\eta$ until it reaches a state $s\in u$. Then, our algorithm takes $\eta_u=\eta_{\tilde{\pi}}$. The only exception is $u_0$, for which we take $\eta_{u_0}=\eta$.
%%Then, our algorithm only constructs $\eta_u$ once it has constructed an augmented path $\tilde{\rho}$ that terminates in $u$ (i.e., $u_k=u$);


%$u'$ (without violating safety) when the initial state is sampled from $\eta_u$ and the policy used is $\pi_{e}$---i.e.,
%\begin{align*}
%    \Pr[e\mid\eta_u] = \Pr_{s\sim\eta_u, \zeta\sim\D_{\pi_e}}[\zeta\models e\mid s_0=s].
%\end{align*}

%Now, given an augmented path $\tilde{\rho}$, we describe how to construct a sequence of state distributions $\eta_0,\ldots,\eta_{k}$ such that $\eta_i$ is a distribution over $u_i$. We do so inductively. First, for $u_0$, we take $\eta_0 = \eta$. For the inductive case, we use:
%\begin{definition}
%\label{def:induceddistribution}
%\rm
%Given an edge $e=u\to u'$, initial state distribution $\eta_u$ over states $s\in u$, and policy $\pi_e$, the \emph{successor state distribution} $\eta[\pi_e,\eta_u]$ is the probability distribution over $u'$ such that for a set of states $S'\subseteq u'$, the probability of $S'$ according to $\eta[\pi_e,\eta_u]$ is defined to be
%\begin{align*}
%\Pr_{s\sim\eta[\pi_e,\eta_u]}[s\in S'] = \Pr_{s_0\sim\eta_u, \zeta\sim\D_{\pi_e,s_0}}\left[s_{i(\zeta,e)}\in S'\mid \zeta\models e\right].
%\end{align*}
%\end{definition}
%Intuitively, $\eta[\pi_e,\eta_u]$ is the state distribution induced by using $\pi_e$ from $s\sim\eta_u$ until we reach a state $s'\in u'$. Finally, continuing our construction of $\eta_i$, we take
%\begin{align}\label{eqn:statedistribution}
%\eta_{i+1} = %\eta[\pi_i,\eta_i]\qquad(\forall i>0). 
%\end{align}

%\textbf{Final policy.}
%
%Once our algorithm has processed a final subgoal region $u$, it trains a final policy $\pi_u$ for $u$ and returns $\tilde{\pi}=(\tilde{\rho}_u,\pi_u)$.


%Then, the cost of the newly discovered path from $u_0$ to $u_2$ via $u_1$ is $c_{u_1} -\log(p)$. If this is less that every known existing path to $u_2$, $c_{u_2}$ is updated and $\eta_{u_2}$ is taken to be the distribution $\eta[u_1\to u_2, \eta_{u_1}]$.

%Furthermore, our algorithm maintains the known minimum cost $c_u$ to each subgoal region $u$ from $u_0$.



% This optimization objective corresponds to the reinforcement learning objective of the MDP $\M' = (S, A, P, T, \eta_{u_1})$ with rewards given by $R(\zeta) = \mathbbm{1}(\zeta\models(u_1,u_2))$. In order to effectively apply existing reinforcement learning algorithms we might need to provide shaped rewards corresponding to this objective (We discuss how we can automatically shape rewards when abstract graphs are generated from \toolname specifications later).

%After learning a policy for the edge $u_1\to u_2$, the algorithm samples trajectories using $\pi_{u_1\to u_2}$ and initial state distribution $\eta_{u_1}$ to estimate the probability $p = P(u_1\to u_2;\eta_{u_1})$ that $u_2$ is reached without violating safety.







==> checklist.tex <==
% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{In the supplement.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In the supplement.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{We compare sample-efficiency which is independent of the platform on which the algorithms are run.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{All assets are open source and available under the MIT licence.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{URL to repository is provided.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
